SLO beyond the Hardware Isolation Limits

Performance isolation is a keystone for SLO guarantees with shared resources in cloud and datacenter environments. To meet SLO requirements, the state of the art relies on hardware QoS support (e.g., Intel RDT) to allocate shared resources such as last-level caches and memory bandwidth for co-located latency-critical applications. As a result, the number of latency-critical applications that can be deployed on a physical machine is bounded by the hardware allocation capability. Unfortunately, such hardware capability is very limited. For example, Intel Xeon E5 v3 processors support at most four partitions for last-level caches, i.e., at most four applications can have dedicated resource allocation. This paper discusses the feasibility and unexplored challenges of providing SLO guarantees beyond the limits of hardware capability. We present CoCo to show the feasibility and the benefits. CoCo schedules applications to time-share interference-free partitions as a transparent software layer. Our evaluation shows that CoCo outperforms non-partitioned and round-robin approaches by up to 9x and 1.2x.

==> 006-conclusion.tex <==
\section{Conclusion}

In this paper, we explore the feasibility and the benefit of providing SLO guarantee beyond the hardware limits.
We propose CoCo, a coordinated container scheduler with dynamic time-sharing resource partitioning for performance-aware workload consolidation.
CoCo dynamically analyzes application characteristics, adjusting the resource time-sharing weights, and scheduling applications with the MQ-WRR algorithm.
It enables the support for multiple LC applications with limited number of CLOSs.
Our evaluation demonstrates the effectiveness of CoCo in that it improves the maximum load retainment by up to 920\% and 17\%, compared with non-partitioned and the round-robin approaches, respectively.
Continuing on this work, future research includes workload-aware CLOS configuration, capacity upper bound inference and thus admission control, and so on.
% In the future, we plan to add the online admission control to the implementation so that capacity upper-bound detection can be done at runtime.
% Instead of blindly accepting new application workloads to consolidate (which leading to SLO violations for both old and new workloads), CoCo will reject the container creation commands.
% until capacity is below the upper-bounds.
% In addition, as workflows in microservices or FaaS generally have data or execution dependencies, multiple containers of the same microservices can be potentially put in one CLOS to save limited CLOS.

==> discarded.tex <==
\begin{figure*}[!ht]
    \centering
    \subfigure[LLC contention on Memcached]{\includegraphics[scale=0.28]{figs/fig-llc-memcached.pdf}}\quad
    \subfigure[LLC contention on Nginx]{\includegraphics[scale=0.28]{figs/fig-llc-nginx.pdf}}\quad
    \subfigure[LLC contention on MongodB]{\includegraphics[scale=0.28]{figs/fig-llc-mongodb.pdf}}
    \subfigure[Memory contention on Memcached]{\includegraphics[scale=0.28]{figs/fig-mem-memcached.pdf}}\quad
    \subfigure[Memory contention on Nginx]{\includegraphics[scale=0.28]{figs/fig-mem-nginx.pdf}}\quad
    \subfigure[Memory contention on MongodB]{\includegraphics[scale=0.28]{figs/fig-mem-mongodb.pdf}}
    \caption{Sensitivity of Different Applications to Resource Contention}
    \label{fig:sensitivity}
\end{figure*}

% talk about sensitivity to different resource contention injection
\textbf{Sensitivity to Resource Contention.}
During the experiments, we progressively increase the intensity of each type of shared resource contention, and evaluate the performance degradation of each application.
An intensity value of zero means that the contention injector is not running.
An intensity value of ten is the largest resource contention injected to the services:
(a) for LLC, it means that threads are created to issue random access that covers the size of the LLC;
(b) for memory bandwidth, it means that threads are created to access a small portion of the memory (e.g, 10\%, to decouple the effects of contention in memory bandwidth from contention in memory capacity) so that the memory bandwidth is saturated.
When one service is running, there is no other workloads running but only the contention injector.
Therefore, we can conclude that the performance degradation is caused purely by the generated shared resource contention.

Figure \ref{fig:sensitivity} shows some of the results on the impact of gradually increased shared resource interference (LLC and memory bandwidth) on the latency (including the 50th, 99th, 99.9th percentiles) for Memcached, Nginx, and MongoDB, respectively.
We summarizes several key observations from the characterization of the above workloads:
\begin{itemize}
    \item Shared resource interference has more impact on the tail latency than the median or mean latency. For example, LLC and memory bandwidth interference has negligible effect on the 50th percentile latency (blue lines), compared to the 99\% latency (red lines) and 99.9\% latency (yellow lines). However, service-level objectives (SLOs) are typically targeting tail latencies.
    \item Each service has different sensitivities to different types of shared resource contention. For example, Memcached is more sensitive to LLC interference, as it has more server performance degradation when facing LLC contention compared to memory contention. Nginx, on the other hand, does not behave differently under LLC or memory contention.
    \item Different services have different sensitivities to the same type of shared resource contention. For example, under LLC interference, the 99th percentile latency of Memcached is 8x of the 50th percentile latency, while the 99th percentile latency of Nginx is 28x of the 50th percentile latency.
    Different services have different behaviors at tail. In Memcached, the 99\% tail latency is significantly different from the 99.9\% tail latency. However, in MongoDB, the two tail latencies are nearly the same. 
\end{itemize}

==> dropped-challenges.tex <==
\section{Challenges}
\label{sec:challenges}

\tianyin{Note that the challenges need to be ``addressed'' otherwise they should not appear here. The current writing does not tell me how do you address the challenges. If they are not addressed, they should be moved into a discussion section. Note that the current writing, even they are addressed, is better be merged into Section 4.}

This section describes the two major challenges we identified when designing CoCo to deal with the limitations imposed by CAT/MBA.

% talk about CAT and MBA conflicts
\noindent
\textbf{Conflicts between Intel CAT and MBA.}
Although Intel CAT and MBA provide trustworthy partition of LLC and memory bandwidth to each CLOS, there may be conflicts when configuring CAT and MBA at the same time.
Since MBA uses a programmable rate controller between the cores and the interconnect, LLC and memory controller, bandwidth to LLC may also be reduced when reducing memory bandwidth using MBA.
For instance, the effect of increasing the bit length of the capacity bit-mask for \texttt{CLOS1} has a higher chance to be canceled out by setting a lower throttling value for \texttt{CLOS1}.
Therefore, it is hard to throttle memory-bandwidth-intense applications which also uses the off-core caches effectively.

% Therefore, CoCo always increase or decrease memory bandwidth together with LLC capacity.
% Otherwise, throttling bandwidth-intense applications which also use the off-core caches will be compromised by increasing memory bandwidth but decreasing LLC capacity.
% As Figure \ref{fig:e2e} shows, CoCo achieves 29\% improvement by monotonically configuring CAT and MBA.

% talk about context switch overheads (mostly cache flushing overheads)
\noindent
\textbf{Cache Misses After CLOS Migration.}
Once a set of CLOSs are configured by setting the bit-masks, the hardware will get the hint on how to partition the cache space for each CLOS.
After a change of CLOS configuration, the changed cache space ($\Delta C$ in terms of cache ways) will be added to or removed from the CLOS.
However, the cached pages in the cache space $\Delta C$ will not be flushed, which limits the new owner of the CLOS (which $\Delta C$ belongs to) from using the newly allocated cache space.
Similarly, a change of CLOS-process association has the same problem.
For instance, \texttt{CLOS-A} and \texttt{CLOS-B} own cache partition $C_a$ and $C_b$ respectively.
After a configuration change, \texttt{CLOS-A} owns $C_b$ and \texttt{CLOS-B} owns $C_a$.
But cache hits from \texttt{CLOS-A} can still lead to access to $C_a$, which no longer owned by \texttt{CLOS-A} and thus limits the usage of $C_a$ by \texttt{CLOS-B} (leading to more cache misses).
If the access frequency from \texttt{CLOS-A} is high, the least-frequently-used cache replacement policy does not help with CLOS migration.

% Therefore, CoCo flushes and invalidates the cache in the original cache partition for each CLOS after each configuration change by paying up to 6.1\% overhead (recall Section \ref{sec:eval-e2e}) of warming up cache.

%%%%%%

% % talk about CAT and MBA conflicts
% \textbf{Conflicts between Intel CAT and MBA.}
% Although Intel CAT and MBA provide trustworthy partition of LLC and memory bandwidth to each CLOS, there may be conflicts when configuring CAT and MBA at the same time.
% Since MBA uses a programmable rate controller between the cores and the interconnect, LLC and memory controller, bandwidth to LLC may also be reduced when reducing memory bandwidth using MBA.
% Therefore, CoCo always increase or decrease memory bandwidth together with LLC capacity.
% Otherwise, throttling bandwidth-intense applications which also use the off-core caches will be compromised by increasing memory bandwidth but decreasing LLC capacity.
% As Figure \ref{fig:e2e} shows, CoCo achieves 29\% improvement by monotonically configuring CAT and MBA.

% % talk about context switch overheads (mostly cache flushing overheads)
% \textbf{CLOS Migration Overheads.}
% Once a set of CLOSs are configured by setting the bit masks, the hardware will know how to partition the cache space for each CLOS.
% After a change of configuration, cache space (in terms of cache ways) will be added to or removed from each CLOS.
% However, the cache in the original cache space will be not flushed, which limits the usage of cache space of the new owner CLOS.
% For instance, CLOS-A and CLOS-B own cache partition $C_a$ and $C_b$ respectively.
% After a configuration change, CLOS-A owns $C_b$ and CLOS-B owns $C_a$.
% But cache hits from CLOS-A can still lead to access to $C_a$, which no longer owned by CLOS-A and thus limits the usage of $C_a$ by CLOS-B (leading to more cache misses).
% If the access frequency from CLOS-A is high, the cache replacement policy does not help with CLOS migration.
% Therefore, CoCo flushes and invalidates the cache in the original cache partition for each CLOS after each configuration change by paying up to 6.1\% overhead (recall Section \ref{sec:eval-e2e}) of warming up cache.
